TDCOSMO XV: Population Analysis of Lines of Sight of 25 Strong Galaxy-Galaxy Lenses with Extreme Value Statistics

Time-Delay Cosmography is a technique for measuring $H_0$ with strong gravitational lensing. It requires a correction for line of sight perturbations, and it is necessary to build tools to assess populations of these lines of sight efficiently. We aim demonstrate the techniques necessary to analyze line of sight effects at a population level, and investigate whether strong lenses fall in preferably overdense environments. We analyze a set of 25 galaxy-galaxy lens lines of sight in the Strong Lensing Legacy Survey sample using standard techniques, then perform a hierarchical analysis to constrain the population-level parameters. We introduce a new statistical model for these posteriors that may provide insight into the underlying physics of the system. We find the median value of $\kappa_{\rm{ext}}$ in the population model to be $0.033 \pm 0.010$. The median value of $\kappa_{\rm{ext}}$ for the individual lens posteriors is $0.008 \pm 0.015$. Both approaches demostrate that our systems are drawn from an overdense sample. The different results from these two approaches show the importance of population models that do not multiply the effect of our priors.

==> tables/SL2S_Sample_old.tex <==
\begin{table}
\begin{tabular}{lrrrrrrrr}
\toprule
Name & RA (deg) & Dec (deg) & $z_d$ & $z_s$ & $\mu_{bf}$ & $\xi_{bf}$ & $log(\sigma_{bf})$ & $\kappa_{med}$ \\
\midrule
SL2SJ0214-0405 & 33.547 & -4.084 & 0.609 & 1.880 & -0.001 & 0.179 & -3.686 & 0.008 \\
SL2SJ0217-0513 & 34.405 & -5.225 & 0.646 & 1.850 & 0.027 & 0.206 & -3.260 & 0.041 \\
SL2SJ0219-0829 & 34.759 & -8.493 & 0.389 & 2.150 & 0.005 & 0.128 & -3.542 & 0.015 \\
SL2SJ0225-0454 & 36.296 & -4.909 & 0.238 & 1.200 & -0.010 & 0.083 & -4.235 & -0.005 \\
SL2SJ0226-0420 & 36.544 & -4.337 & 0.494 & 1.230 & -0.014 & 0.184 & -4.383 & -0.010 \\
SL2SJ0232-0408 & 38.215 & -4.140 & 0.352 & 2.340 & -0.000 & 0.091 & -3.515 & 0.010 \\
SL2SJ0849-0412 & 132.290 & -4.207 & 0.722 & 1.540 & 0.001 & 0.258 & -3.825 & 0.008 \\
SL2SJ0901-0259 & 135.275 & -2.985 & 0.670 & 1.190 & -0.006 & 0.102 & -4.178 & -0.000 \\
SL2SJ0904-0059 & 136.033 & -0.998 & 0.611 & 2.360 & 0.009 & 0.120 & -3.326 & 0.022 \\
SL2SJ1359+5535 & 209.957 & 55.597 & 0.783 & 2.770 & -0.006 & 0.218 & -3.270 & 0.008 \\
SL2SJ1405+5243 & 211.443 & 52.720 & 0.526 & 3.010 & -0.003 & 0.139 & -3.210 & 0.011 \\
SL2SJ1411+5651 & 212.904 & 56.855 & 0.322 & 1.420 & 0.006 & 0.163 & -3.917 & 0.013 \\
SL2SJ1420+5630 & 215.249 & 56.502 & 0.483 & 3.120 & -0.025 & 0.121 & -3.294 & -0.012 \\
SL2SJ1427+5516 & 216.880 & 55.279 & 0.511 & 2.580 & -0.007 & 0.172 & -3.441 & 0.004 \\
SL2SJ2203+0205 & 330.871 & 2.089 & 0.400 & 2.150 & 0.001 & 0.092 & -3.552 & 0.012 \\
SL2SJ0212-0555 & 33.199 & -5.931 & 0.750 & 2.740 & 0.018 & 0.031 & -3.202 & 0.033 \\
SL2SJ0218-0802 & 34.505 & -8.047 & 0.884 & 2.060 & -0.003 & 0.057 & -3.738 & 0.006 \\
SL2SJ0220-0949 & 35.192 & -9.824 & 0.572 & 2.610 & 0.017 & 0.002 & -3.356 & 0.029 \\
SL2SJ0233-0438 & 38.280 & -4.644 & 0.671 & 1.870 & -0.007 & 0.153 & -3.726 & 0.002 \\
SL2SJ0848-0351 & 132.197 & -3.851 & 0.682 & 1.550 & 0.026 & 0.176 & -3.286 & 0.040 \\
SL2SJ0855-0147 & 133.917 & -1.792 & 0.365 & 3.390 & -0.018 & 0.124 & -3.073 & -0.002 \\
SL2SJ1404+5200 & 211.227 & 52.007 & 0.456 & 1.590 & -0.011 & 0.117 & -4.114 & -0.005 \\
SL2SJ1406+5226 & 211.710 & 52.439 & 0.716 & 1.470 & -0.005 & 0.155 & -4.021 & 0.001 \\
SL2SJ2205+0147 & 331.279 & 1.784 & 0.476 & 2.530 & 0.007 & 0.146 & -3.045 & 0.024 \\
SL2SJ2221+0115 & 335.453 & 1.262 & 0.325 & 2.350 & 0.027 & 0.117 & -3.217 & 0.042 \\
\bottomrule
\end{tabular}
\caption{Basic information and final best fit parameters for the population of lenses in our sample. }
\label{table:lens_table}
\end{table}
